Exact recovery in Gaussian weighted stochastic block model and planted dense subgraphs: Statistical and algorithmic thresholds

In this paper, we study the exact recovery problem in the Gaussian weighted version of the Stochastic block model with two symmetric communities. We provide the information-theoretic threshold in terms of the signal-to-noise ratio (SNR) of the model and prove that when SNR $<1$, no statistical estimator can exactly recover the community structure with probability bounded away from zero. On the other hand, we show that when SNR $>1$, the Maximum likelihood estimator itself succeeds in exactly recovering the community structure with probability approaching one. Then, we provide two algorithms for achieving exact recovery. The Semi-definite relaxation as well as the spectral relaxation of the Maximum likelihood estimator can recover the community structure down to the threshold value of 1, establishing the absence of an information-computation gap for this model. Next, we compare the problem of community detection with the problem of recovering a planted densely weighted community within a graph and prove that the exact recovery of two symmetric communities is a strictly easier problem than recovering a planted dense subgraph of size half the total number of nodes, by establishing that when the same SNR$< 3/2$, no statistical estimator can exactly recover the planted community with probability bounded away from zero. More precisely, when $1 <$ SNR $< 3/2$ exact recovery of community detection is possible, both statistically and algorithmically, but it is impossible to exactly recover the planted community, even statistically, in the Gaussian weighted model. Finally, we show that when SNR $>2$, the Maximum likelihood estimator itself succeeds in exactly recovering the planted community with probability approaching one. We also prove that the Semi-definite relaxation of the Maximum likelihood estimator can recover the planted community structure down to the threshold value of 2.

==> S1_abstract.tex <==

\begin{abstract}
In this paper,  we first analyze the exact recovery problem in the Gaussian weighted version of the Stochastic block model with two symmetric communities. We provide the information-theoretic threshold in terms of the signal-to-noise ratio (SNR) of the model and prove that when $\text{SNR} <1$, no statistical estimator can exactly recover the community structure with probability approaching one. On the other hand, we show that when $\text{SNR} >1$, the Maximum likelihood estimator itself succeeds in exactly recovering the community structure with probability approaching one. Then, we provide two algorithms for achieving exact recovery. The Semi-definite relaxation as well as the spectral relaxation of the  Maximum likelihood estimator can recover the community structure down to the threshold value of $1$, establishing the absence of an information-computation gap for this model.
\par 
Next, we compare the problem of community detection with the problem of recovering a planted densely weighted community within a graph and prove that the exact recovery of two symmetric communities is a strictly easier problem than recovering a planted dense subgraph of size half the total number of nodes, by establishing that when the same $\text{SNR} < \frac{3}{2}$, no statistical estimator can exactly recover the planted community with probability approaching one. More precisely, when $ 1 <\text{SNR} < \frac{3}{2}$ exact recovery of community detection is possible, both statistically and algorithmically, but it is impossible to exactly recover the planted dense community, even statistically, in the Gaussian weighted model.   Finally, we show that when $\text{SNR} >2$, the Maximum likelihood estimator itself succeeds in exactly recovering the planted community with probability approaching one. We also prove that the Semi-definite relaxation of the  Maximum likelihood estimator can recover the planted community structure down to the threshold value of $2$.
\end{abstract}

==> S2_introduction.tex <==
\section{Introduction and related works} \label{sec:intro}
Learning community structures in graphs is a central problem in computer science,  statistical machine learning, and complex networks. The stochastic block model (SBM) functions as a random graph model wherein distinct groups of vertices exhibit varied connectivity patterns. This model has been extensively studied as a standard framework for investigating clustering and community detection (See \cite{goldenberg2009survey}).  Furthermore, it serves as a rich domain for exploring the intricate tradeoffs between information and computation inherent in combinatorial statistics and the broader field of data science. We refer the reader to \cite{abbe2023community}, \cite{moore2017computer}  for more details. 

  \subsection{Gaussian weighted stochastic block model: description}
  The stochastic block model is a random graph model with community structures \cite{HOLLAND1983109}, \cite{abbe2023community}. In the symmetric two community case, the random graph $G_n = ([n], E_n)$ with vertex set $[n]:=\{1, 2, \cdots, n-1, n\}$ and edge set $E_n \subset  \binom{[n]}{2}:= \{\{i,j\}: i \neq j \in [n]\}$ has two equally sized clusters given by $\sigma^* \in \{\pm 1\}^{n}$   ($n$ even) such that $ \{i \in [n]: \sigma_i =1\} = \{ i\in [n]: \sigma_i =-1\} =\frac{n}{2}. $
  
  The vertices connect with probability $p$ within clusters and $q$ across clusters. The problem of exact recovery asks to output a balanced partition $\hat{\sigma}$ that recovers the unobserved partition $\sigma^*$  correctly with probability approaching one as $n \to  \infty$.  Indeed, one can only hope to recover the communities up to a global sign flip of the labels. It turns out that the critical scaling of the parameters for this problem is given by the following for constants $a, b > 0$
  \begin{equation} \label{def:CritSBM0}
  p=\frac{a \log n}{n}  \text{ and } q = \frac{b \log n}{n}.
  \end{equation}
   In the Gaussian weighted version of the Stochastic block model (GWSBM), we denote a weighted graph $G_{n} \sim$ SBM$(n, \mu_1\,\mu_2, \tau^2)$ on $n$ vertices with labels $(\sigma_i^*)_{i\in [n]}$ such that  
   $\#\{i\in [n]: \sigma_i^*=1\}=\#\{i\in [n]: \sigma_i^*=-1\}=\frac{n}{2}$ and conditioned on this labeling $(\sigma_i^*)_{i\in [n]}$,  we have  Gaussian\footnote{$ N(\mu, \tau^2):= \text{Normally distributed random variable with mean } \mu \text{ and variance } \tau^2$} weighted edges sampled independently for every pair $\{i,j\}$.
   \begin{equation}\label{def:GWSBM0}
A_{ij}=A_{ji} \sim
\begin{cases}
  N(\mu_1, \tau^2)  & \text{if } \sigma^*(i) =\sigma^*(j)  \\
   N(\mu_2, \tau^2) & \text{if }  \sigma^*(i)\neq \sigma^*(j) 
\end{cases}
   \end{equation} 
   
     We focus on the assortative case $\mu_1>\mu_2$,   work with the critical scaling of  $\mu_1$ and $\mu_2$ and for $\alpha >\beta $ and $ \tau >0$ constants, we define the signal-to-noise ratio (SNR)  as
    \begin{equation} \label{def:CritGWSBM0}
     \mu_1= \alpha \sqrt{\frac{\log n}{n}}, \quad   \mu_2= \beta\sqrt{\frac{\log n}{n}} \quad \text{and} \quad \text{SNR}:= \frac{(\alpha -\beta)^2}{8\tau^2}.
    \end{equation}

 The problem of exact recovery asks to recover the planted community labeling $(\sigma_i^*)_{i\in [n]}$ exactly up to a global sign flip, having observed an instance of the weighted graph $G_n\sim$ SBM$(n, \mu_1\,\mu_2, \tau^2)$ or equivalently a sample of the random $n \times n $ symmetric weighted adjacency matrix $(A_{ij})_{i,j,\in [n]}$ of the graph. 
 Let us  denote the parameter space $\Theta_n$  with 
 $\mathbf{1}_n := (1, \cdots, 1)\in \mathbb{R}^n$ as
 \begin{equation}
 \Theta_n = \{\sigma\in \{\pm1\}^n, \langle\sigma, \mathbf{1}_n\rangle=0\}.
 \end{equation}
 
  We define the agreement ratio between $\hat{\sigma},  \sigma  \in \{\pm 1\}^n$ as  
  \[
  M(\hat{\sigma}, \sigma)= \max \left(\frac{1}{n}\sum_{i=1}^n \mathbf{1}_{\hat{\sigma}(i)=\sigma(i)}, \frac{1}{n}\sum_{i=1}^n \mathbf{1}_{-\hat{\sigma}(i)=\sigma(i)}\right).
  \]


Then, we say that the problem of exact recovery is solvable if having observed an instance of the weighted random graph $G_n \sim$ SBM$(n,\mu_1, \mu_2,\tau^2)$ with an unobserved $\sigma^* \in \Theta_n$, we output a community label $\hat{\sigma} \in \Theta_n
$ such that  $\mathbb{P} \left[M(\hat{\sigma},\sigma^*)=1\right] \to 1.$ We say the problem of exact recovery is unsolvable otherwise. That is, with probability bounded away from zero, every estimator fails to exactly recover the community labels, as the number of vertices grows.
\subsection{Gaussian weighted stochastic block model:  results and proof sketch}
In this section, we present our results along with the ideas of the proof for GWSBM in comparison with the breakthrough works of \cite{abbe2014exact}, \cite{Mossel_2016}, \cite{hajek2016achieving}, \cite{abbe2019entrywise} that established an important set of results for the SBM to inspire a Gaussian weighted version. Detailed proofs of all the theorems and lemmas are provided in the appendix.  
\par 
The literature for community detection and related problems is vast, and weighted version similar to ours have been considered in the literature  \cite{7447159}, \cite{jog2015informationtheoretic}, \cite{xu2018optimal}. More precisely, results similar to Theorems \ref{thm:Negative0}, and \ref{thm: Positive0} has been established in  \cite{esmaeili2021community} under certain assumptions. \cite{bandeira2015random} established a result similar to Theorem \ref{thm:SDP0} for the $\mathbb{Z}_2$ synchronization problem, using a different semi-definite program \ref{eq:SDP0}.
\par
To explore the information-theoretic limits, we start by examining the maximum a posteriori (MAP) estimation, designed to maximize the probability of accurately reconstructing communities. In the context of uniform community assignment, (which is the case for us as we are fixing an unknown community labeling $\sigma^*$ with balanced community sizes, which could be chosen uniformly from all the possible $\binom{n}{\frac{n}{2}}$ choices of community assignments), MAP estimation is equivalent to maximum likelihood estimation (MLE). We refer to \cite{abbe2023community}[Section 3.1] for more details.
\par 
Next, we observe that the MLE for SBM and GWSBM  is given by the following.
    \begin{equation} \label{eq:MLE0}
   \hat{\sigma}_{MLE}= \underset{\sigma \in \Theta_n}{ \argmax} \hspace{.1 cm}f_A(\sigma):=\sum_{i,j} A_{ij}\sigma_i \sigma_j 
    \end{equation}
    
Under the critical scaling \ref{def:CritSBM0} in the stochastic block model,  it was shown in \cite{abbe2014exact} that if $|\sqrt{a} -\sqrt{b}| <\sqrt{2}$ then MLE fails to exactly recover the true community structure $\sigma^*$ with probability bounded away from zero as $n\to \infty$. 
In the Gaussian weighted version of the stochastic block model \ref{def:GWSBM0} we establish the following statistical impossibility result.
\begin{theorem}[\textbf{Statistical impossibility of exact recovery}] \label{thm:Negative0}
     Let $G_n \sim $ SBM$(n,\mu_1, \mu_2, \tau^2)$ with $\mu_1, \mu_2$ in the critical scaling regime \ref{def:CritGWSBM0}, and $\alpha > \beta$, $\tau >0$ be constants. If SNR$<1$ then MLE fails in recovering the community label $\sigma^*$ bounded away from zero. 
     \[ \underset{n \to \infty}{\limsup}\hspace{.1cm}\p(M(\hat{\sigma}_{MLE}, \sigma^*)=1) < 1 \leftrightarrow \underset{n \to \infty}{\liminf}\hspace{.1cm}\p(M(\hat{\sigma}_{MLE}, \sigma^*)\neq 1) > 0.\]
\end{theorem}

 We prove this by establishing that whenever SNR$<1$, with probability approaching one we can find vertices $i$ and $j$ in each community such that swapping them increases the likelihood \ref{eq:MLE0} and hence causes MLE to fail to recover the ground truth $\sigma^*$ exactly. Without loss of generality, we assume that the planted community is given by $\sigma^* =(1, \cdots, 1, -1, \cdots, -1) \in \Theta_n$, and $G_n \sim $ SBM$(n, \mu_1, \mu_2, \tau^2)$ conditioned on $\sigma^*$. We denote the resulting communities  as
    \[C_+=\left\{1, \cdots, \frac{n}{2}\right\},  \quad C_{-}=\left\{\frac{n}{2}+1, \cdots, n\right\}.\]
    
    More precisely, we define the set of bad pairs of vertices in $G_n$ with $\sigma^*[i\leftrightarrow j]$ denoting the vector obtained by swapping the values of coordinates $i$ and $j$ in $\sigma^*$.
    \begin{equation}\label{def:bad0}
    \mathcal{B}(G_n) := \{(i,j): i\in C_+, j\in C_{-}, f_A(\sigma^*)\leqslant f_A(\sigma^*[i\leftrightarrow j])\}.
    \end{equation}
    
    


From \ref{eq:MLE0} we observe that  $f_A(\sigma^*)\leqslant f_A(\sigma^*[i\leftrightarrow j]) $ is the same as the event that the likelihood of the partition $\sigma^*[i\leftrightarrow j]$ is larger than the planted one $\sigma^*$. So it reduces to the following.
\begin{lemma}
   MLE fails to solve the exact recovery with probability bounded away from zero if $\mathcal{B}(G_n)$ is non-empty with probability bounded away from zero. More precisely, we have the following
   \begin{equation} \label{eq:NegLB0}
   \underset{n \to \infty}{\liminf}\hspace{.1cm}\p(M(\hat{\sigma}_{MLE}, \sigma^*)\neq1) \geqslant \frac{1}{2} \underset{n \to \infty}{\liminf}\hspace{.1cm} \p (\mathcal{B}(G_n)\neq \emptyset)
   \end{equation}
\end{lemma}
We now analyze the condition $f_A(\sigma^*)\leqslant f_A(\sigma^*[i\leftrightarrow j])$ and show that  $\underset{n \to \infty}{\lim}\hspace{.1cm}\p (\mathcal{B}(G_n)\neq \emptyset) =1.$
\begin{definition}
    For a vertex $i \in C_+$, and $j \in C_-$ we define the following.
    \[
    d_+(i)= \sum_{v\in C_+}A_{iv}, \quad  d_+(j)=  \sum_{v\in C_-}A_{jv}, \quad d_-(i)= \sum_{v\in C_-}A_{iv},
    \]
    \[
    d_-(j)=  \sum_{v\in C_+}A_{jv}, \quad d_-(i\setminus j)=\sum_{v\in C_- \setminus j}A_{iv}, \quad  d_-(j\setminus i)=\sum_{v\in C_+ \setminus i}A_{jv}
    \]
\end{definition}
It is worth observing that $d_+(i)$ and $ d_+(j)$ sums the edge weights that $i$ and $j$ have with their own communities $C_+$ and  $C_-$, and $d_-(i)$ and $ d_-(j)$ sums the edge weights that $i$ and $j$ have with their opposite communities $C_-$ and  $C_+$ respectively.  With the notations above we have the following local condition for a bad pair $\{i,j\}$.
\begin{lemma}
 Let $i\in C_+, j\in C_-$. Then we have the following equivalence.
    \[
    f_A(\sigma^*)\leqslant f_A(\sigma^*[i\leftrightarrow j]) \leftrightarrow  d_+(i)+d_+(j) \leqslant d_-(i\setminus j)+d_-(j\setminus i).
    \]
\end{lemma}

Finally, we analyze $\mathcal{B}(G_n)$ \ref{def:bad0} the set of bad pairs of vertices by analyzing sets $\mathcal{B}_+(G_n)$  and $ \mathcal{B}_-(G_n)$ with individual vertices satisfying certain conditions, and apply the first and second-moment methods \cite{10.5555/3002498}. We now define the following sets with diverging constants $c_n \to \infty $ to be chosen later according to the proof.

\begin{definition}  The set of bad vertices (instead of bad pairs) in each community in $G_n$ is given by
\[
\mathcal{B}_+(G_n):=\left\{i: i \in C_+, d_{+}(i) \leqslant d_{-}(i)-c_n\right\}, 
\]
\[
\mathcal{B}_-(G_n):=\left\{j: j \in C_-, d_{+}(j) \leqslant d_{-}(j)-c_n\right\},
\]
\end{definition}

 \begin{lemma} \label{lem:Bto10}
     With the notations above, if $\mathcal{B}_+(G_n)$ and $\mathcal{B}_-(G_n)$ are non-empty with probability approaching $1$, then $\mathcal{B}(G_n)$ is non-empty with probability approaching  $1$ as $n \to  \infty$.
\end{lemma}

It remains to establish that if SNR$<1$, we have  $\mathbb{P}\left[ \mathcal{B}_+(G_n)\neq \emptyset \right] = \mathbb{P}\left[ \mathcal{B}_-(G_n)\neq \emptyset \right]=1 - o(1)$.
\begin{lemma} \label{lem:SM0}
 If $\text{SNR}<1$, then $\mathcal{B}_+(G_n)$ and  $\mathcal{B}_-(G_n)$ are non empty with probability approaching $1$.
\[
  \mathbb{P}\left[ \mathcal{B}_+(G_n)\neq \emptyset \right]  = 
  \mathbb{P}\left[ \mathcal{B}_-(G_n)\neq \emptyset \right]=1 - o(1).
\]
\end{lemma}
We now apply the second-moment method to the  random variable $Z_+ = \sum_{i \in C_+}\mathbf{1}_{d_{+}(i) \leqslant d_{-}(i)-c_n}$.
\[
\mathbb{P}\left[ \mathcal{B}_+(G_n)\neq \emptyset \right]  =\mathbf{P}[Z_+ \geqslant 1] \geqslant \frac{\mathbb{E}\left[Z_+\right]^2}{\mathbb{E}\left[Z_+^2\right]}
\]

With this lower bound on the probability, it reduces to proving the following two limits.
\begin{equation}
n \mathbb{P}\left[ d_+(1) \leqslant d_-(1) -c_n\right] \to \infty,
\end{equation}
\begin{equation}
\frac{\mathbb{P}\left[d_+(1) \leqslant d_-(1) -c_n \cap d_+(2) \leqslant d_-(2) -c_n\right]}{\mathbb{P}\left[d_+(1) \leqslant d_-(1) -c_n\right] \mathbb{P}\left[d_+(1) \leqslant d_-(1) -c_n\right]}  \to 1 .
\end{equation}


\begin{lemma} We observe that the following holds whenever SNR$<1$.
\[
n \mathbb{P}\left[ d_+(1) \leqslant d_-(1) -c_n\right]  =  n \mathbb{P}\left[N(0,1) \geqslant 
     (1+o(1)) \frac{(\alpha - \beta)\sqrt{\log n}}{2\tau}\right] = n^{1 -\text{SNR} +o(1)} \to  \infty
\]
\end{lemma}

Finally, we prove that the events $E_1 =\{d_+(1) \leqslant d_-(1) -c_n\}$ and $E_2= \{ d_+(2) \leqslant d_-(2) -c_n\}$ are asymptotically independent,  and  for notational purposes we define $a_n \sim b_n$ if $\lim_{n \to \infty} \frac{a_n}{b_n}=1$. 
\begin{lemma} Let $Z_1, Z_2,$ and $ Z$ be IID $N(0,1)$ random  variables, and $s= \frac{\alpha -\beta}{2\tau}$. Then we have
\begin{align}
\frac{\mathbb{P}\left[E_1 \cap E_2\right]}{\mathbb{P}\left[E_1\right] \mathbb{P}\left[E_2\right]}
\sim \frac{\mathbb{P}\left[Z_1 \geqslant s\sqrt{\log n} +\frac{Z}{\sqrt{n-2}}\cap Z_2 \geqslant s\sqrt{\log n} +\frac{Z}{\sqrt{n-2}}\right]}{\mathbb{P}\left[Z_1 \geqslant s\sqrt{\log n} +\frac{Z}{\sqrt{n-2}}\right] \mathbb{P}\left[Z_1 \geqslant s\sqrt{\log n}+\frac{Z}{\sqrt{n-2}}\right]} \sim 1
\end{align}
\end{lemma}

The proof of the two lemmas above and hence the proof of Theorem \ref{thm:Negative0} depends on the fact that $d_+(1\setminus2), d_+(2\setminus 1), A_{12}, d_-(1), d_-(2)$ are jointly independent collections of random variables and satisfy the following distributional identities.
\[
d_+(1\setminus2):= \sum_{i\in C_+ \setminus 2}A_{i1} \overset{d}{=}N\left(\left(\frac{n}{2}-2\right)\mu_1, \left(\frac{n}{2}-2\right)\tau^2\right),
\]
\[
d_+(2\setminus1):= \sum_{i\in C_+ \setminus 1}A_{i2} \overset{d}{=}N\left(\left(\frac{n}{2}-2\right)\mu_1, \left(\frac{n}{2}-2\right)\tau^2\right),
\]
\[
d_-(1)=\sum_{j\in C_-}A_{1j}\overset{d}{=} N\left(\frac{n}{2}\mu_2, \frac{n}{2}\tau^2\right), \quad
d_-(2)=\sum_{j\in C_-}A_{2j} \overset{d}{=} N\left(\frac{n}{2}\mu_2, \frac{n}{2}\tau^2\right).
\]

Now, we turn towards proving statistical possibility results. Under the critical scaling \ref{def:CritSBM0} in SBM, it was proven in \cite{abbe2014exact}  if $|\sqrt{a} -\sqrt{b}| >\sqrt{2}$ then MLE can exactly recover the true community structure $\sigma^*$ with probability approaching one as $n\to \infty$. In the Gaussian weighted version of the stochastic block model \ref{def:GWSBM0} we establish the following statistical possibility result. 
\begin{theorem}[\textbf{Statistical possibility of exact recovery}] \label{thm: Positive0}
    Let  $G_n \sim$ SBM$(n, \mu_1, \mu_2, \tau^2)$ \ref{def:GWSBM0}. Then MLE can recover the  $\sigma^*$ whenever $\text{SNR} >1$. More precisely, $ \mathbb{P}\left[M(\hat{\sigma}_{\text{MLE}}, \sigma^*)= 1\right] \to 1$ if $\text{SNR} >1$.
\end{theorem}

The proof of this theorem relies on analyzing the inequality $f_A(\hat{\sigma}) \geqslant f_A(\sigma^*)$ 
 and observing that  MLE \ref{eq:MLE0} fails to recover the true community labels $\sigma^*$ with probability approaching $1$ if and only if there exists $ \hat{\sigma}$ such that $f_A(\hat{\sigma}) \geqslant f_A(\sigma^*)$. For a subset of vertices $S_+ \subseteq C_+$ and $S_- \subseteq C_-$ we define 
\[
d_+(S_+) =\sum_{i \in S_+, k \in C_+\setminus S_+}A_{ik}, \quad 
d_+(S_-) =\sum_{j \in S_-, l \in C_-\setminus S_-}A_{jl}
\]
\[
d_-(S_+\setminus S_-) =\sum_{i \in S_+, j \in C_-\setminus S_-}A_{ij}, \quad 
d_-(S_-\setminus S_+) =\sum_{j \in S_-, i \in C_+\setminus S_+}A_{ij}
\]

 \begin{lemma} $\exists$ $\hat{\sigma} \in \Theta_n$ such that  
     $f_A(\hat{\sigma}) \geqslant f_A(\sigma^*)$  $\smallimplies$ $\exists  S_+ \subseteq C_+, S_- \subseteq C_-$ such that $|S_+|=|S_-|$ and  
     \begin{equation} \label{eq:Pos0}
     d_+(S_+) +d_+(S_-)\leqslant  d_-(S_+\setminus S_-) +d_-(S_-\setminus S_+).
     \end{equation} 
 \end{lemma}
 We simply use union bound to prove that MLE \ref{eq:MLE0}  solves exact recovery \ref{thm: Positive0} as soon as \text{SNR} $>1$  by proving that such events of the kind \ref{eq:Pos0} occur with probability approaching zero. We define
 \[
 E:=\{\exists S_+ \subseteq C_+, S_- \subseteq C_- : |S_+|=|S_-|, d_-(S_-\setminus S_+) + d_-(S_+ \setminus S_-) \geqslant d_+(S_+)+d_-(S_-) \} =\cup_{k=1}^{\frac{n}{4}}E_k
 \]
 \[
 E_k= \{\exists S_+ \subseteq C_+, S_- \subseteq C_- : |S_+|=|S_-| =k, d_-(S_-\setminus S_+) + d_-(S_+ \setminus S_-) \geqslant d_+(S_+)+d_-(S_-)\}
 \]
 \begin{lemma} With the notations above, if SNR$>1$ then $\mathbb{P}\left[E\right] =  \mathbb{P}\left[\cup_{k=1}^{\frac{n}{4}}E_k \right] \leqslant \sum_{k=0}^{\frac{n}{4}}\mathbb{P}\left[E_k\right] \to 0$.
 \end{lemma}
 The proof of this lemma relies on that $ d_-(S_-\setminus S_+), d_-(S_+ \setminus S_-), d_+(S_+), d_-(S_-)$ are jointly independent random variables satisfying the following distributional identities.
     \[
     d_+(S_+)\overset{d}{=}  N( k(n/2 -k) \mu_1, k(n/2 -k) \tau^2), \quad 
     d_+(S_-)\overset{d}{=}  N( k(n/2 -k) \mu_1, k(n/2 -k) \tau^2)
     \]
     \[
     d_-(S_+\setminus S_-) \overset{d}{=} N( k(n/2 -k) \mu_2, k(n/2 -k) \tau^2), \quad
     d_-(S_-\setminus S_+) \overset{d}{=} N( k(n/2 -k) \mu_2, k(n/2 -k) \tau^2)
     \]
     
      If SNR$>1$, we have the following for $k=1$ with $\text{SNR}= 1+2\delta$ for some $\delta >0$.
     \[
     \mathbb{P}\left[E_1\right] \leqslant  \frac{n^2}{4}  \mathbb{P}\left[ N(0,1) \geqslant \sqrt{(n/2 -1)} \left(\frac{\mu_1- \mu_2}{\tau}\right)\right] \leqslant \frac{n^2}{4}  e^{-\frac{2 
     (n -2)  \text{SNR}\log  n}{n}}  = \frac{1}{4}  \frac{1}{n^{4\delta + o(1)}} \to 0.
     \]

 we observe that MLE \ref{eq:MLE0} is a discrete optimization problem over an exponential-sized solution space and not a polynomially tractable problem in the worst-case sense, and also in the approximate-case sense \cite{doi:10.1137/050640904}. So, we look for potential algorithmic solutions to recover the ground truth $\sigma^*$. Under the critical scaling \ref{def:CritSBM0} in SBM it was proven in \cite{hajek2016achieving} that a semi-definite relaxation (SDP) of MLE \ref{eq:MLE0} solves exact recovery if $|\sqrt{a} -\sqrt{b}| > \sqrt{2}$. In the GWSBM \ref{def:GWSBM0}, we establish the following algorithmic possibility result whenever SNR$> 1$.
       To start, we observe that MLE \ref{eq:MLE0} can be rewritten as the following problem.
\begin{equation} \label{def:MLE0R}
\max_{Y, \sigma} \langle A, Y \rangle : Y = \sigma \sigma^T, \, Y_{ii} = 1, \, i \in [n], \, \langle \mathbf{J}, Y \rangle = 0. 
\end{equation}

 $Y = \sigma \sigma^T$ is a rank-one positive semi-definite matrix. Relaxing this condition by dropping the rank-one restriction, we obtain the following convex relaxation of \ref{def:MLE0R}:
\begin{equation} \label{eq:SDP0}
\hat{Y}_{\text{SDP}} = \arg\max_{Y} \langle A, Y \rangle : Y \succeq 0, \, Y_{ii} = 1, \, \langle \mathbf{J}, Y \rangle = 0.
\end{equation}


Let $Y^*=\sigma^*\sigma^{*^{\top}}$ and $\mathcal{Y}_n \triangleq\left\{\sigma \sigma^{\top}: \sigma \in\{-1,1\}^n, \langle \sigma ,\mathbf{1}\rangle =0\right\}$. The following result establishes the algorithmic tractability of the exact recovery problem under the  SDP procedure.

\begin{theorem}[\textbf{Semi-definite relaxation achieves exact recovery}]\label{thm:SDP0}
Let $G_n \sim$ SBM$(n, \mu_1, \mu_2, \tau^2)$. 
 \[
 \text{ If  SNR }  >1  \text{ then  } \min _{Y^* \in \mathcal{Y}_n} \mathbb{P}\left\{\hat{Y}_{\mathrm{SDP}}=Y^*\right\}\to  1  \hspace{.1 cm} \text{ as } \hspace{.1 cm} n \rightarrow \infty.
 \]
\end{theorem}

Following \cite{hajek2016achieving} we prove the theorem by first producing a deterministic sufficient condition for SDP to achieve exact recovery. Let $\mathbf{J}$ denote an $n \times n$ matrix with all entries equal to $1$ and $\lambda_2 (S)$ denote the second smallest eigenvalue of a symmetric $n \times n$ matrix $S$.
\begin{lemma}
 Suppose  $ \exists$ $D^{*}=\operatorname{diag}\left\{d_{i}^{*}\right\}$ with $\{d^*_i\}_{i=1}^{n} \in \mathbb{R}^n$ and $\lambda^{*} \in \mathbb{R}$ such that 
 \begin{equation} \label{eq:DualCert0}
  S^{*} := D^{*}-A+\lambda^{*} \mathbf{J} \hspace{.1 cm} \text{satisfies} \hspace{.1 cm}  S^{*} \succeq 0, \lambda_{2}\left(S^{*}\right)>0, \hspace{.1 cm} \text{and} \hspace{.1 cm} S^{*} \sigma^{*}=0.
 \end{equation}
 
Then SDP recovers the true solution. More precisely, $\widehat{Y}_{\mathrm{SDP}}=Y^{*}$ is the unique solution to \ref{eq:SDP0}.
\end{lemma}

The proof of this lemma follows from the weak duality of semi-definite programming, and now we make a clever choice of $D^*$ and $\lambda^*$ such that $S^*$ satisfies all the conditions above \ref{eq:DualCert0} with probability approaching one.
More precisely, for all $1\leqslant i \leqslant n$ we take $d_{i}^{*}=\sum_{j=1}^{n} A_{i j} \sigma_{i}^{*} \sigma_{j}^{*}$ and choose $\lambda^{*}= \frac{\mu_1+\mu_2}{2}$.  By definition of $S^*= D^* -A+\lambda^*\mathbf{J}$ with $D^*$ and $\lambda^*$ as above, we have $S^*\sigma^* = 0$, and it reduces to proving the following.
\begin{equation}\label{eq:SDPMain0}
  \mathbb{P}\left[S^* \succeq 0\cap \lambda_2(S^{*})>0\right] =\mathbb{P}\left[\inf _{x \perp \sigma^{*},\|x\|=1} \langle x, S^{*} x \rangle >0\right] \to 1
\end{equation}

Simplifying the quantity $\langle x, S^{*} x \rangle$ requires us to prove the following.
\begin{equation}
  \mathbb{P}\left[ \min _{i \in[n]} d_{i}^{*}+\mu_1 -\|A-\mathbb{E}[A]\| >0\right] \to  1
\end{equation}

From  bounds  on norms of Gaussian random matrices \cite{Vershynin_2018}, we have  for an absolute constant $c >0$ $\mathbb{P}\left[\|A-\mathbb{E}[A]\| \geqslant 3\tau\sqrt{n}\right] \leqslant 2e^{-cn} $. Therefore, it is enough to prove the following 
\begin{equation}
    \mathbb{P}[ \min _{i \in[n]} d_{i}^{*}> 4\tau\sqrt{n}] =  \mathbb{P}[ \cap_{i=1}^{n} \{d_{i}^{*}> 4\tau\sqrt{n}\}] \to  1
\end{equation}

We prove this using a union bound argument and observing that  for all $1\leqslant i \leqslant n$
\[
d_{i}^*=\sum_{j=1}^{n} A_{i j} \sigma_{i}^{*} \sigma_{j}^{*} \overset{ d}{=} N\left(\left(\frac{n}{2}-1\right)\mu_1, \left(\frac{n}{2}-1\right)\tau^2\right) - N\left(\frac{n}{2}\mu_2, \frac{n}{2}\tau^2\right),
\]
\[
\implies \sum_{i=1}^{n} \mathbb{P}\left[ d^*_i \leqslant 4\tau \sqrt{n} \right] = n \mathbb{P}\left[ d^*_i \leqslant 4\tau \sqrt{n} \right] \leqslant \frac{1}{n^{\text{SNR} -1 +o(1)}} \to  0.
\]

\par
This proves that there is no information computation gap \cite{bandeira2018notes} in this model as SDP \ref{eq:SDP0} achieves exact recovery until the statistical threshold produced by  MLE \ref{eq:MLE0}. We end the analysis of this model  \ref{def:GWSBM0} by proving that even spectral relaxation of MLE \ref{eq:MLE0} achieves exact recovery until the same threshold.  In SBM, it was proven in \cite{abbe2019entrywise} that a spectral relaxation of MLE \ref{eq:MLE0} solves exact recovery whenever $|\sqrt{a} -\sqrt{b}| > \sqrt{2}$.  In the Gaussian weighted version of the stochastic block model \ref{def:GWSBM0}, we establish the following algorithmic possibility result.
\begin{theorem}[\textbf{Spectral relaxation achieves exact recovery}] \label{thm:Spec0}
    Let $G_n \sim$ SBM$(n, \mu_1, \mu_2, \tau^2)$  with the assumption that $A_{ii} \overset{IID}{\sim} N(\mu_1, \tau^2)$.  Let $B:=  A - \frac{n (\mu_1 +\mu_2)}{2} \frac{\mathbf{1}_n}{\sqrt{n}}\frac{\mathbf{1}_n}{\sqrt{n}}^{\top}$. If $\text{SNR}$ $>1$  then $\hat{\sigma}:= \text{sign} (u_1)$ achieves exact recovery where $u_1$ is the eigenvector corresponding to the largest eigenvalue $\lambda_1$ of $B$. More precisely, if \text{SNR} $>1$ then $\mathbb{P} \left[ M(\hat{\sigma}, \sigma^*) =1\right] \to 1$.
\end{theorem}
 The proof of this theorem is based on a more general spectral separation result obtained in \cite{abbe2019entrywise}[Theorem 1.1] and we defer the detailed proof of the above result in the appendix. Now we analyze a Gaussian weighted planted dense subgraph model of linear proportional size.
\subsection{Gaussian weighted planted dense subgraph model: description}
In comparison to the SBM, the binary version of the planted dense subgraph problem \cite{ariascastro2013community} 
has a single  (denser) cluster of size $\gamma n$ for  $\gamma \in (0,1)$, and vertices within the planted community connect with probability $p$ and every other pair connect with probability $q$.
In the Gaussian weighted planted dense subgraph model (GWPDSM) denoted as PDSM$(n, \mu_1,\mu_2, \tau^2)$ we have a weighted graph $G_{n}$ on $n$  vertices with binary labels $(\zeta_i^*)_{i\in [n]}$ such  that  
\[
\#\{i\in [n]: \zeta_i^*=1\}= \gamma n, \quad 
\#\{i\in [n]: \zeta_i^*=0\}= (1-\gamma) n
\] 

and conditioned on this labeling $(\zeta_i^*)_{i\in [n]}$, for each pair  $\{i,j\}$, we have a weighted edge 
\begin{equation}\label{def:GWPDSM0}
A_{ij}=A_{ji} \sim
\begin{cases}
  N(\mu_1, \tau^2) & \text{if } \zeta^*(i) =\zeta^*(j) =1   \\
   N(\mu_2, \tau^2) & \text{otherwise}   
\end{cases}
\end{equation} 

sampled independently for every distinct pair $\{i,j\}$.  To simplify the writing, we focus on the assortative case, $\mu_1>\mu_2$ with the critical scaling \ref{def:CritGWSBM0}  of $\mu_1= \alpha \sqrt{\frac{\log n}{n}}, \mu_2= \beta\sqrt{\frac{\log n}{n}}.$ We further have our SNR  given by $\text{SNR}:= \frac{(\alpha -\beta)^2}{8\tau^2}$ with $\alpha >\beta $ and $ \tau >0$ constants.
\par
 The problem of exact recovery of the densely weighted community asks to recover the planted community labeling $(\zeta_i^*)_{i\in [n]}$ exactly having observed an instance of the weighted graph $G_n\sim$ PDSM$(n, \mu_1\,\mu_2, \tau^2)$. Let us  denote the parameter space $\Theta^{\gamma}_n$ with
 $\mathbf{1}_n := (1, \cdots, 1)\in \mathbb{R}^n$ as 
 \begin{equation} \label{eq:SOL1}
 \Theta^{\gamma}_n = \{\zeta\in \{0, 1\}^n, \langle\zeta, \mathbf{1}_n\rangle=\gamma n\},
 \end{equation}
 
 We define the agreement ratio between  $\hat{\zeta},  \zeta  \in \{0, 1\}^n$ as     $M(\hat{\zeta}, \zeta)= \frac{1}{n}\sum_{i=1}^n \mathbf{1}_{\hat{\zeta}(i)=\zeta(i)} $.

Then, we say that the problem of exact recovery is solvable if having observed an instance of the weighted random graph $G_n \sim$ PDSM$(n,\mu_1, \mu_2,\tau^2)$ with an unobserved $\zeta^* \in \Theta^{\gamma}_n$, we output a community label $\hat{\zeta} \in \Theta^{\gamma}_n $ such that $\p (M(\hat{\zeta},\zeta^*)=1) \to 1.$  We say the problem of exact recovery is unsolvable otherwise. That is, with probability bounded away from zero, every estimator fails to exactly recover the densely weighted community, as the number of vertices grows.
\subsection{Gaussian weighted planted dense subgraphs: results and proof sketch}
 In this section, we present our results along with the ideas of the proof for GWPDSM in comparison with the works \cite{hajek2016achieving} \cite{hajek2016achieving1} that established an important set of results for the binary version. Detailed proofs of all the theorems and lemmas are provided in the appendix.
 \par
 To explore information theoretic limits, we analyze the maximum likelihood estimator (MLE).
 \vspace{-0.4 em}
\begin{equation} \label{eq:MLEPDSM0}
   \hat{\zeta}_{MLE}= \underset{\zeta \in \Theta^{\gamma}_n}{ \argmax} \hspace{.1 cm}g_A(\zeta):=\sum_{i,j} A_{ij}\zeta_i \zeta_j 
   \vspace{-0.4 em}
\end{equation}

Under the critical scaling \ref{def:CritSBM0} in the binary version, it was proven in \cite{hajek2016achieving} that below a certain threshold, exact recovery of the planted community is not solvable. In particular, MLE \ref{eq:MLEPDSM0} fails to recover the ground truth $\zeta^*$ with probability bounded away from zero as $n \to  \infty$. In GWPDSM \ref{def:GWPDSM0} we establish the following statistical impossibility result.
\begin{theorem}[\textbf{Statistical impossibility of exact recovery of the planted community}] \label{thm:Negative1'}
      With parameter $\gamma \in  (0,1)$ let $G_n \sim $ PDSM$(n, \mu_1, \mu_2, \tau^2)$  and with critical scaling \ref{def:CritGWSBM0}.
      If  $\gamma$ SNR$<\frac{3}{4}$ then MLE fails in recovering the community label $\zeta^*$ bounded away from zero. 
     \[ 
     \underset{n \to \infty}{\limsup}\hspace{.1cm}\p(M(\hat{\zeta}_{MLE}, \zeta^*)=1) < 1 \leftrightarrow \underset{n \to \infty}{\liminf}\hspace{.1cm}\p(M(\hat{\zeta}_{MLE}, \zeta^*)\neq 1) > 0.
     \]
\end{theorem}
  We prove this by establishing that whenever $\gamma$SNR$<\frac{3}{4}$, with probability approaching one we can find a vertex $i$ in the planted community and a vertex $j$ from the rest such that swapping them increases the likelihood \ref{eq:MLEPDSM0} and hence causes MLE to fail to recover the ground truth $\zeta^*$ exactly. Without loss of generality, we assume that the planted community is given by $\zeta^* =(\mathbf{1}_{\gamma n}, \mathbf{0}_{(1-\gamma)n}) \in \Theta_n^{\gamma}$, and $G_n \sim $ PDSM$(n, \mu_1, \mu_2, \tau^2)$ conditioned on $\zeta^*$. We denote the planted community  as
    \[C^* := \left\{ i \in [n]: \zeta_i^*=1\right\}=\left\{1, \cdots, \gamma n\right\}, \quad
    [n] \setminus C^*:=\left\{\gamma n +1, \cdots, n\right\}.\]
    \vspace{-1cm}
    \begin{definition} 
       We define the set of bad pairs of vertices in $G_n$ with $\zeta^*[i\leftrightarrow j]$ denoting the vector obtained by swapping the values of coordinates $i$ and $j$ in $\zeta^*$.
    \begin{equation} \label{def:Bad1}
    \mathcal{C}(G_n) := \{(i,j): i\in C^*, j\in [n] \setminus C^*, g_A(\zeta^*)\leqslant g_A(\zeta^*[i\leftrightarrow j])\},
    \end{equation}
\end{definition}

From \ref{eq:MLEPDSM0} we observe that $g_A(\zeta^*)\leqslant g_A(\zeta^*[i\leftrightarrow j]) $ is the same as the event that the likelihood of the partition $\zeta^*[i\leftrightarrow j]$ is larger than the planted one $\zeta^*$. So it reduces to the following.
\begin{lemma}
   MLE fails to solve the exact recovery with probability bounded away from zero if $\mathcal{C}(G_n)$ is non-empty with probability bounded away from zero. More precisely, we have the following 
   \[
   \underset{n \to \infty}{\liminf}\hspace{.1cm}\p(M(\hat{\zeta}_{MLE}, \zeta^*)\neq1) \geqslant \frac{1}{2} \underset{n \to \infty}{\liminf}\hspace{.1cm} \p (\mathcal{C}(G_n)\neq \emptyset)
   \]
\end{lemma}
We analyze $g_A(\zeta^*)\leqslant g_A(\zeta^*[i\leftrightarrow j]) $ and show that 
$\underset{n \to \infty}{\lim}\hspace{.1cm}\p (\mathcal{C}(G_n)\neq \emptyset) =1.$
\begin{definition}
    For a vertex $i \in C^*$, and $j \in [n]\setminus C^*$ we define the following.
    \[
    e(i, C^*) = \sum_{ k \in C^*} A_{ik} =e(i, C^* \setminus \{i\}), \quad 
    e(j, C^* \setminus \{i\}) = \sum_{ k \in C^*  \setminus \{i\}} A_{jk}
    \]
\end{definition}
It is worth observing that $e(i, C^*)$  sums the edge weights that $i $ has with $C^*$.
\begin{lemma}
With the notations above and $i \in C^*$, and $j \in [n]\setminus C^*$ we have the following.
    \[
    g_A(\zeta^*)\leqslant g_A(\zeta^*[i\leftrightarrow j]) \leftrightarrow  e(i, C^*) \leqslant e(j, C^* \setminus \{i\}).
    \]
\end{lemma}  

With the lemma above we apply the second-moment method to $Z = \sum_{ i \in C^*, j \in [n]\setminus C^*} Z_{ij}$ with
\begin{equation}
Z_{ij}=\mathbf{1}_{\mathcal{C}_{ij}}
\quad \text{with} \quad 
\mathcal{C}_{ij} : =\{e(i, C^*) \leqslant e(j, C^*\setminus \{i\})\}
\end{equation}
\begin{equation}
\mathcal{C}(G_n) =\{(i,j): i \in C^*, j \in [n]\setminus C^*, e(i, C^*)\leqslant e(j,C^*\setminus \{i\})\} = \cup_{ i \in C^*, j \in [n]\setminus C^* } \mathcal{C}_{ij}.
\end{equation}

We have $\mathbb{P}\left[\mathcal{C}(G_n) \neq \emptyset\right] =\mathbb{P}\left[Z \geqslant 1\right]$ and it reduces to proving $\mathbb{P}\left[Z \geqslant1 \right] \to 1$ if $ \gamma \text{SNR} <\frac{3}{4}$. Applying the second-moment method to $Z$ it further reduces to proving the following two limits.
\begin{equation}
  \sum_{(i,j) \in C^* \times [n]\setminus C^*} \mathbb{P}\left[\mathcal{C}_{ij}\right]\to \infty
  \end{equation}
  \begin{equation} \label{eq:SMC'}
   \frac{\sum_{(i_1, j_1) \neq (i_2, j_2)   \in  C^* \times [n]\setminus C^*} \mathbb{P}\left[ \mathcal{C}_{(i_1, j_1)}\cap \mathcal{C}_{(i_2, j_2)}\right]}{\left(\sum_{(i,j) \in C^* \times [n]\setminus C^*} \mathbb{P}\left[\mathcal{C}_{ij}\right]\right)^2} \to 1 .
  \end{equation}
\begin{lemma} \label{lem:First1'}
 Let $C = C(\alpha, \beta, \gamma, \tau): = \frac{\gamma (1- \gamma )\tau \sqrt{2} }{(\alpha -\beta) \sqrt{2\pi \gamma }} $. If $ \gamma \text{SNR} < 1$ then for $Z,Z_1$ IID $N(0,1)$    we have
\begin{equation} \label{eq:First1'}
\sum_{(i,j) \in C^* \times [n]\setminus C^*} \mathbb{P}\left[\mathcal{C}_{ij}\right] \sim  \gamma (1-\gamma)n^2 \mathbb{P}\left[ \left\{Z_1  \geqslant \frac{Z}{ \sqrt{2\gamma n -3}} + s \sqrt{\log n}\right\}\right] \sim C \frac{n^{2(1-\gamma \text{SNR})}}{\sqrt{\log n}} \to \infty.
\end{equation}
\end{lemma}
 The proof relies on that fact that $e(i, C^*)$ and $e(j, C^* \setminus \{i\})$ are independent and  we have 
 \begin{equation}
 e(i, C^*) \overset{d}{=} N((\gamma n -1)\mu_1,(\gamma n -1)\tau^2), \quad 
 e(j, C^*\setminus \{i\}) \overset{d}{=} N((\gamma n -1)\mu_2,(\gamma n -1)\tau^2)
 \end{equation}
\begin{lemma} \label{lem:Second1'}
If $ \gamma \text{SNR} <  \frac{3}{4}$ then, we have the following   
\[
\frac{\sum_{(i_1, j_1) \neq (i_2, j_2)   \in  C^* \times [n]\setminus C^*} \mathbb{P}\left[ \mathcal{C}_{(i_1, j_1)}\cap \mathcal{C}_{(i_2, j_2)}\right]}{\left(\sum_{(i,j) \in C^* \times [n]\setminus C^*} \mathbb{P}\left[\mathcal{C}_{ij}\right]\right)^2} \to 1 
\]
\end{lemma}
The proof builds on the fact that for $i_1 \neq i_2 \in C^* $ and $j_1 \neq j_2 \in [n] \setminus C^*$ we have   $e_{i_1, i_2}, e(i_1, C^* \setminus \{i_2\}), e(i_2, C^* \setminus \{i_1\}),  e(j_1, C^* \setminus \{i_1\}), e(j_2, C^* \setminus \{i_2\})$ are jointly independent Gaussians with
\[
e(i_1, C^* \setminus \{i_2\}) \overset{d}{=} N( (\gamma n -2)\mu_1, (\gamma n-2) \tau^2), \quad
e(i_2, C^* \setminus \{i_1\}) \overset{d}{=} N( (\gamma n -2)\mu_1, (\gamma n-2) \tau^2)
\]
\[
e(j_1, C^* \setminus \{i_1\}) \overset{d}{=}  N( (\gamma n -1)\mu_2, (\gamma n-1) \tau^2), \quad
e(j_2, C^* \setminus \{i_2\}) \overset{d}{=} N( (\gamma n -1)\mu_2, (\gamma n-1) \tau^2)
\]

\begin{lemma}
Let  $Z_1, Z_2,$ and $ Z$ be IID $N(0,1)$ with $s=\frac{ (\alpha -\beta) \sqrt{\gamma}}{\tau \sqrt{2}}$. For $i_1\neq i_2 \in C^*, j_1\neq j_2 \in [n]\setminus C^*$
    \begin{equation}\label{eq:SM1'}
\frac{\mathbb{P}[\mathcal{C}_{(i_1, j_1)}\cap \mathcal{C}_{(i_2, j_2)}]}{\mathbb{P}[\mathcal{C}_{i_1,j_1}]\mathbb{P}[\mathcal{C}_{i_1,j_1}]} \sim  \frac{\mathbb{P}  \left[ \left\{Z_1  \geqslant \frac{Z}{ \sqrt{2\gamma n -3}} + s \sqrt{\log n}\right\} \cap  \left\{Z_2  \geqslant \frac{Z}{ \sqrt{2\gamma n -3}} + s \sqrt{\log n}\right\} \right]}{\mathbb{P}  \left[ Z_1  \geqslant \frac{Z}{ \sqrt{2\gamma n -3}} + s \sqrt{\log n}\right] \mathbb{P}  \left[Z_2  \geqslant \frac{Z}{ \sqrt{2\gamma n -3}} + s \sqrt{\log n}\right]} \sim 1 
   \end{equation}
\end{lemma}
 So, leading term  in \ref{eq:SMC'} is   $\sum_{i_1 \neq i_2  \in  C^*,j_1\neq  j_2 \in [n]\setminus C^*} \mathbb{P}\left[ \mathcal{C}_{(i_1, j_1)}\cap \mathcal{C}_{(i_2, j_2)}\right] \sim \left(\sum_{(i,j) \in C^* \times [n]\setminus C^*} \mathbb{P}\left[\mathcal{C}_{ij}\right]\right)^2.$ It is rather surprising that the subleading orders in the sum \ref{eq:SMC'} does  go to zero only if $\gamma \text{SNR} < \frac{3}{4}$.
\[
\frac{\sum_{i_1 =i_2  \in  C^*,j_1\neq  j_2 \in [n]\setminus C^*} \mathbb{P}\left[ \mathcal{C}_{(i_1, j_1)}\cap \mathcal{C}_{(i_2, j_2)}\right]}{\left(\sum_{(i,j) \in C^* \times [n]\setminus C^*} \mathbb{P}\left[\mathcal{C}_{ij}\right]\right)^2} 
\sim
\frac{\mathbb{P}\left[  \mathcal{C}_{(i, j_1)}\cap \mathcal{C}_{(i, j_2)}\right]}{ \gamma n \mathbb{P}\left[\mathcal{C}_{ij}\right]^2} 
\sim
0  \quad ( \text{if} \hspace{.1 cm} \gamma \text{SNR} < \frac{3}{4})
\]
\[
\frac{\sum_{i_1 \neq i_2  \in  C^*,j_1 =  j_2 \in [n]\setminus C^*} \mathbb{P}\left[ \mathcal{C}_{(i_1, j_1)}\cap \mathcal{C}_{(i_2, j_2)}\right]}{\left(\sum_{(i,j) \in C^* \times [n]\setminus C^*} \mathbb{P}\left[\mathcal{C}_{ij}\right]\right)^2}
\sim
\frac{\mathbb{P}\left[  \mathcal{C}_{(i_1, j)}\cap \mathcal{C}_{(i_2, j)}\right]}{(1-\gamma )n \mathbb{P}\left[\mathcal{C}_{ij}\right]^2}  \sim
0 \quad (\text{if} \hspace{.1 cm} \gamma \text{SNR} < \frac{3}{4})
\]

 This is because for $i \in C^*$ and $j_1 \neq j_2 \in [n] \setminus C^*$ or $i_1 \neq i_2 \in C^*$ and $j \in [n] \setminus C^*$ we have  \footnote{$ \Phi(z) = \p [N(0,1) \geqslant z] =\int_{z}^{\infty} \phi(t) dt 
 \text{  with  } \phi(t) =\frac{1}{\sqrt{2\pi}}e^{-\frac{t^2}{2}}$} \footnote{ $a_n \simeq b_n \implies a_n \leqslant \text{ poly }(\log n) b_n  \text{  and  } b_n \leqslant \text{ poly } (\log n) a_n $}
 \begin{align*}
 \frac{\mathbb{P}[\mathcal{C}_{(i, j_1)}\cap \mathcal{C}_{(i, j_2)}]}{n \p [\mathcal{C}_{ij}]^2}
 \sim 
 \frac{\mathbb{P}[\mathcal{C}_{(i_1, j)}\cap \mathcal{C}_{(i_2, j)}]}{n \p [\mathcal{C}_{ij}]^2} 
 &
 \sim
 \frac{\mathbb{P}  \left[ \left\{Z_1 \geqslant Z + s\sqrt{2 \log n}  \right\} \cap \left\{Z_2 \geqslant  Z + s\sqrt{2 \log n} \right\} \right]}{n \mathbb{P}  \left[ Z_1 \geqslant Z + s\sqrt{2 \log n}\right]^2 } 
 \\
 &
 \sim 
 \frac{\int_{\mathbb{R}} \Phi^2(z +s\sqrt{2 \log n}) \phi(z) dz}{ n \left(\frac{1}{ s \sqrt{\log n}}\phi (s \sqrt{\log n})\right)^2} 
 \hspace{.1 cm} 
 \simeq
  n^{\frac{4 \gamma \text{SNR}}{3} -1} 
 \to 0
 \end{align*}
 
 Now, we turn towards proving statistical possibility results. In Gaussian weighted planted dense subgraph model \ref{def:GWPDSM0} we establish the following statistical possibility result if $\gamma$SNR$>1$.
 \begin{theorem}[\textbf{Statistical possibility of exact recovery}] \label{thm: Positive1'}
    Let $G_N\sim$  PDSM$(n, \mu_1, \mu_2, \tau^2)$ \ref{def:GWPDSM0}, MLE can exactly recover  $\zeta^*$ as soon as $ \gamma \text{SNR} >1$. More precisely, $ \mathbb{P}\left[M(\hat{\zeta}_{\text{MLE}}, \zeta^*)= 1\right] \to 1$.
\end{theorem}
The proof of this theorem relies on analyzing the inequality $g_A(\hat{\zeta}) \geqslant g_A(\zeta^*)$ and observing that  MLE \ref{eq:MLEPDSM0} fails to recover  $\zeta^*$ with probability approaching $1$ if and only if there exists $ \hat{\zeta} \in \Theta_n^{\gamma}$ such that $g_A(\hat{\zeta}) \geqslant g_A(\zeta^*)$.
For  subsets of vertices $A,B \subseteq [n]$ with $A\cap B = \emptyset$ we define the following
\[
e(A, B) =\sum_{p \in A,q \in B} A_{pq}, \quad 
e(A) = \sum_{p \in A, q \in A} A_{pq}.
\]
\begin{lemma} $\exists$ $\hat{\zeta} \in \Theta_n^{\gamma}$ with  
     $g_A(\hat{\zeta}) \geqslant g_A(\zeta^*)$  $\smallimplies$ $\exists  S_+ \subseteq C^*, S_- \subseteq [n] \setminus C^*$ such that $|S_+| =|S_-|$ and 
     \begin{equation} \label{eq:Pos1'}
     e(S_-) +
     e(C^* \setminus S_+ , S_-) \geqslant 
     e(S_+)+
     e(C^* \setminus S_+, S_+)
     \end{equation} 
 \end{lemma}
 
 We now prove that MLE \ref{eq:MLEPDSM0} can solve exact recovery \ref{thm: Positive1'} as soon as  $\gamma$ \text{SNR} $>1$  by proving that such events of the kind \ref{eq:Pos1'} occur with probability approaching zero. We define the following events
 \[ E:=\{\exists S_+ \subseteq C^*, S_- \subseteq [n] \setminus C^* : |S_+|=|S_-|, e(S_-) +
     e(C^* \setminus S_+ , S_-) \geqslant 
     e(S_+)+
     e(C^* \setminus S_+, S_+) \} =\cup_{l=1}^{K}E_l
 \]
 \[
 E_l= \{\exists S_+ \subseteq C^*, S_- \subseteq [n] \setminus C^* : |S_+|=|S_-| =l, e(S_-) +
     e(C^* \setminus S_+ , S_-) \geqslant 
     e(S_+)+
     e(C^* \setminus S_+, S_+)\}
 \]
 \begin{lemma}\label{lem:Second2'}
 With the notations above, if $\gamma$ \text{SNR} $>1$ then $\mathbb{P}\left[E\right] =  \mathbb{P}\left[\cup_{l=1}^{K}E_l \right] \leqslant \sum_{l =1}^{K} \mathbb{P}[E_l] \to 0.$
 \end{lemma}
The proof of this lemma follows from observing that  $e(S_-), e(S_+), e(C^* \setminus S_+, S_-),$  and $e(C^*\setminus S_+, S_+)$ are jointly independent random variables with 
     \[
     e(S_+)\overset{d}{=}  N\left( \binom{l}{2} \mu_1, \binom{l}{2} \tau^2\right), \quad 
     e(S_-)\overset{d}{=}  N\left( \binom{l}{2} \mu_2, \binom{l}{2} \tau^2\right)
     \]
     \[
     e(C^*\setminus S_+, S_+) \overset{d}{=} N\left( l(K -l) \mu_1, l(K -l) \tau^2 \right), \quad 
     e(C^*\setminus S_+, S_-) \overset{d}{=} N\left( l(K -l) \mu_2, l(K -l) \tau^2\right).
     \]
     
    From  Gaussian tail bounds \cite{Vershynin_2018} we have  for $l=1$ with $ \gamma \text{SNR}= 1+2\delta$.
     \[ 
     \mathbb{P}\left[E_1\right] \leqslant 
     K(n-K) \frac{1}{n^{ \frac{2(K-1) \text{SNR}}{n}}}\leqslant \gamma (1-\gamma) n^2 n^{-2 \gamma  
       \text{SNR} (1+o(1))} =  \frac{\gamma (1-\gamma)}{n^{4\delta +o(1)} }  \to 0
     \] 
     
     We finish this section by establishing that SDP achieves exact recovery of the planted community as soon as $\gamma $SNR$>1$ in comparison to the work \cite{hajek2016achieving} in the binary version. To start, we observe that MLE \ref{eq:MLEPDSM0} can be rewritten as the following discrete optimization problem.
\begin{equation}\label{eq:MLEPDSM0'}
\max_{Z, \zeta} \hspace{.1 cm} \langle A, Z \rangle :  Z =\zeta \zeta^{\top},  Z_{ii} \leqslant  1, \hspace{.1 cm} \forall 
 \hspace{.1 cm} i \in [n],  Z_{ij} \geqslant  0, \hspace{.1 cm} \forall \hspace{.1 cm} i, j \in[n], \langle\mathbf{I}, Z\rangle=\gamma n,  \langle\mathbf{J}, Z \rangle =\gamma^2 n^2.
\end{equation} 
 $Z=\zeta \zeta^{\top}$ is positive semidefinite and rank-one. Removing the rank-one restriction leads to the following convex relaxation of \ref{eq:MLEPDSM0'}, which is a semidefinite program.
\begin{equation} \label{def:SDPPDSM0}
 \hat{Z}_{\mathrm{SDP}}=\underset{Z}{\arg \max } \langle A, Z\rangle:  Z \succeq 0,  Z_{ii} \leqslant 1, \hspace{.1 cm} \forall \hspace{.1 cm} i \in [n], Z_{ij} \geqslant 0, \hspace{.1 cm} \forall \hspace{.1 cm} i, j \in[n], \langle\mathbf{I}, Z\rangle=\gamma n, \langle\mathbf{J}, Z\rangle=\gamma^2 n^2 .
\end{equation}

Let $Z^*=\zeta^*\zeta^{*^{\top}}$ correspond to the true cluster and define $\mathcal{Z}_n=\left\{\zeta \zeta^{\top}: \zeta \in\{0,1\}^n, \langle \zeta, \mathbf{1} \rangle =\gamma n\right\}$. 
\begin{theorem}[\textbf{Semi-definite relaxation achieves exact recovery}] \label{thm:SDP1'}
    Let $G_n \sim$ PDSM$(n, \mu_1, \mu_2, \tau^2)$  
\[
\text{ with parameter } \gamma \in  (0,1) \text{ If }  \gamma \text{SNR} \hspace{.1 cm}>1  \hspace{.1 cm} \text{then} \hspace{.1 cm}
\min _{Z \in \mathcal{Z}_n} \mathbb{P}\left[\hat{Z}_{\mathrm{SDP}}=Z^*\right]\to 1 \hspace{.1 cm} \text{as} \hspace{.1 cm} n \rightarrow \infty.
\]
\end{theorem} 
Following \cite{hajek2016achieving} we prove this theorem by first producing a deterministic sufficient condition for SDP to achieve exact recovery. Let $\mathbf{I}$ be $n\times n$ identity matrix.
\begin{lemma}\label{lem:DetPDSM0}
 Suppose $\exists$  $D^{*}=\operatorname{diag}\left\{d_{i}^{*}\right\}$ with $\{d^*_i\}_{i=1}^{n} \in  \mathbb{R}_{\geqslant 0}^{n}$,  $B^{*} \in \mathbb{R}^{n\times n}_{\geqslant 0},$    and $\lambda^{*}, \eta^{*} \in \mathbb{R}$ such that 
 \begin{equation}\label{eq:First0}
 S^{*} \triangleq D^{*}-B^{*}-A+\eta^{*} \mathbf{I}+\lambda^{*} \mathbf{J} \hspace{.1 cm} \text{satisfies} \hspace{.1 cm} S^{*} \succeq 0, \lambda_{2}\left(S^{*}\right)>0, \hspace{.1 cm} \text{and}  \hspace{.1 cm}S^{*}  \zeta^{*}  =0,
 \end{equation}
 \begin{equation}\label{eq:Second0}
 \hspace{.1 cm}
d_{i}^{*}\left(Z_{i i}^{*}-1\right)  =0 \quad \forall i, \quad 
B_{i j}^{*} Z_{i j}^{*}  =0 \quad \forall i, j,
 \end{equation}

Then SDP recovers the true solution. More precisely, $\widehat{Z}_{\mathrm{SDP}}=Z^{*}$ is the unique solution to \ref{def:SDPPDSM0}.
\end{lemma}

The proof of this lemma follows from the weak duality of semi-definite programming, and now we make a clever choice of $B^*, D^*$  with  $\lambda^* = \frac{\mu_1+\mu_2}{2}$  and $ \eta^* =2\|A-\mathbb{E}[A]\|$  satisfying all the conditions in  \ref{lem:DetPDSM0} with probability approaching one. We take $D^{*}=\operatorname{diag}\left\{d_{i}^{*}\right\}$ with \footnote{ $A_i$ refers to the $i$th row of A} $d^*_i:= \langle (A-\eta^*\mathbf{I}- \lambda^*\mathbf{J})_i, \zeta^*\rangle \mathbf{1}_{i \in C^*}$ and   $B^{*}_{ij}:
=b_{i}^{*} \mathbf{1}_{\left\{i \notin C^{*}, j \in C^{*}\right\}}+b_{j}^{*} \mathbf{1}_{\left\{i \in C^{*}, j \notin C^{*}\right\}}$ with  $b_{i}^{*} \gamma n :=  \langle (\lambda^* \mathbf{J} -A)_i, \zeta^* \rangle \mathbf{1}_{i \notin C^{*}}.$
\par 
It follows immediately that $d_{i}^{*}\left(Z_{i i}^{*}-1\right)  =0, 
B_{i j}^{*} Z_{i j}^{*}  =0$  $\forall$ $i, j,$ and $S^*\zeta* =0$. It remains to prove 
\[
\min \left(\mathbb{P}\left[\cap_{i \notin C^*} \{b_i^*\geqslant 0\} \right ], \quad  \mathbb{P}\left[\cap_{i \in C^*} \{d_i^*\geqslant 0\}\right], \quad  \mathbb{P}\left[ \{S^* \succeq 0\} \cap \{\lambda_{2}\left(S^{*}\right)>0\}\right] \right)\to 1
\]

We prove this simply using union bound by observing that the following holds.
 \begin{equation}
 d^*_i = X_i - 6\tau \sqrt{n} - \lambda^{*} \gamma n \geqslant 0  \hspace{.1 cm} \forall \hspace{.1 cm}  i \in C^*, \quad 
 b_i^* \gamma n = \lambda^{*} \gamma n - X_i  \geqslant 0 \hspace{.1 cm} \forall \hspace{.1 cm} i \notin C^*
 \end{equation}
 \[ \text{where  } X_i \sim N(\gamma n \mu_1, \gamma n \tau^2) \mathbf{1}_{i \in C^*} +
      N(\gamma n \mu_2, \gamma n \tau^2) \mathbf{1}_{i \notin C^*}\]
      
   We now turn to the comparison of the two models discussed and establish that GWSBM \ref{def:GWSBM0} is a strictly easier problem to solve than GWPDSM \ref{def:GWPDSM0} with parameter $\gamma =\frac{1}{2}$.
\subsection{A comparison of exact recovery in two models and conclusion}
We observed that Theorems \ref{thm:Negative0}, \ref{thm: Positive0}, \ref{thm:SDP0}, \ref{thm:Spec0} obtained for GWSBM \ref{def:GWSBM0} prove that if $\text{SNR} <1$, then the task of exact recovery of two balanced communities is impossible, even statistically. But, as soon as $\text{SNR} >1$,  the task of exact recovery is possible, even algorithmically. On the other hand Theorems \ref{thm:Negative1'}, \ref{thm: Positive1'}, \ref{thm:SDP1'} obtained for GWPDSM (with $\gamma = \frac{1}{2}$) \ref{def:GWPDSM0} prove that whenever $\text{SNR} < \frac{3}{2}$, the task of exact recovery of one planted community of size  $\frac{n}{2}$  is statistically impossible. But, as soon as $\text{SNR} >2$, then the task of exact recovery of one planted community of size $\frac{n}{2}$ is algorithmically possible.  So, when $1<\text{SNR} < \frac{3}{2}$, the problem of exact recovery of two balanced communities is algorithmically solvable, whereas the problem of exact recovery of one planted community of size $\frac{n}{2}$ is even statistically unsolvable. This proves that indeed community detection is a strictly easier problem than the planted dense subgraph model as considered in the models \ref{def:GWSBM0}, \ref{def:GWPDSM0}.
\par
It is also interesting to see the inability of first and second-moment methods to match the upper \ref{lem:Second2'} and lower bounds \ref{lem:Second1'} for the Gaussian weighted planted dense subgraph problem.
